Maximum Weighted Loss Discrepancy

Though machine learning algorithms excel at minimizing the average loss over a population, this might lead to large discrepancies between the losses across groups within the population. To capture this inequality, we introduce and study a notion we call maximum weighted loss discrepancy (MWLD), the maximum (weighted) difference between the loss of a group and the loss of the population. We relate MWLD to group fairness notions and robustness to demographic shifts. We then show MWLD satisfies the following three properties: 1) It is statistically impossible to estimate MWLD when all groups have equal weights. 2) For a particular family of weighting functions, we can estimate MWLD efficiently. 3) MWLD is related to loss variance, a quantity that arises in generalization bounds. We estimate MWLD with different weighting functions on four common datasets from the fairness literature. We finally show that loss variance regularization can halve the loss variance of a classifier and hence reduce MWLD without suffering a significant drop in accuracy.

==> Makefile <==
TEXS=main.tex
ALLTEXS=$(shell ls *.tex)
ALLBIBS=$(shell ls *.bib)
PDFS=$(TEXS:.tex=.pdf)

default:
	pdflatex main
	bibtex main
	#latexmk -pdf main

jacob:
	latexmk -pdf main

all: $(PDFS)

clean:
	-rm *~ $(PDFS) *.aux *.bbl *.blg *.log *.out

%.pdf: $(ALLTEXS) $(ALLBIBS)
	pdflatex $(@:.pdf=.tex)
	bibtex $(@:.pdf=)
	pdflatex $(@:.pdf=.tex)
	pdflatex $(@:.pdf=.tex)

refs:
	@if [ ! -d "refdb" ]; \
	  then \
	  git clone https://github.com/percyliang/refdb;\
	fi
	cd refdb; git pull

run:
	go main.pdf


==> age_example.tex <==
\begin{figure}[t]
\centering
\newcommand{\ssc}{0.7}
\newcommand{\len}{7}
\begin{tikzpicture}[scale=0.5]
\draw[<->] (-1*\len+0.5,0) -- (\len-0.5,0);
\node (n1) at (\len+1.2,0) {\small $x_\text{non-sensitive}$};
\draw[<->] (0,-2) -- (0,\len);
\node (n1) at (0,\len+0.5) {\small $x_\text{sensitive}$};

\foreach \x in {-3,-2,-1,1,2,3}
	\draw (\x,2pt) -- (\x,-2pt) node[anchor=north,scale=\ssc] {$\x$};
\foreach \y in {1,2,3}
	{
	\draw (2pt,\y cm) -- (-2pt,\y cm) node[anchor=east,scale=\ssc] {$\y$};
	\node[scale=1] (p1) at (\y,\y) {$\boldsymbol{+}$};
	\node[scale=1] (p1) at (-1*\y,\y) {$\boldsymbol{-}$};
	}
\node[scale=1] (p1) at (\len-1,\len-1) {$\boldsymbol{+}$};
\node[scale=1] (p1) at (-1*\len+1,\len-1) {$\boldsymbol{-}$};


\draw (2pt,\len-1) -- (-2pt,\len-1) node[anchor=east,scale=\ssc] {$K$};
\draw (\len-1,2pt) -- (\len-1,-2pt) node[anchor=north,scale=\ssc] {$K$};
\draw (-1*\len+1,2pt) -- (-1*\len+1,-2pt) node[anchor=north,scale=\ssc] {$-K$};


\end{tikzpicture}
\caption{\label{fig:age_example} 
	The plot shows some distribution of sensitive and non-sensitive attributes for which coarse loss variance converges very slowly.
	There are same number of positive and negative individuals.
	The non-sensitive attribute of positive individuals is uniformly distributed in $\{1,2,\dots,K\}$, and the non-sensitive attribute of negative individuals is uniformly distributed in $\{-1,-2,\dots,-K\}$.
	The sensitive attribute for both positive and negative individuals is the absolute value of the non-sensitive attribute.
	}
\end{figure}

==> different_loss.tex <==
\begin{table}
	\centering
	\scalebox{0.9}{
	\begin{tabular}{ll}
		\toprule
		\bf Parity & \bf Regularizer \\ \midrule
			Overall misclassification (OM)&  $\var [\ell(h,z)]$\\
		%	Only considering protected groups & $\var [\E [\ell(h,z)\mid A]]$\\
			False positive (FP)&$\var [\ell(h,z) \mid y=0]$\\
			False negative (FN)&$\var [\ell(h,z) \mid y=1]$\\
			%false discovery (FD)&$\var [\ell(h,z) \mid \hat y=1]$\\
			%false omission (FO)&$\var [\ell(h,z) \mid \hat y=0]$\\
			\midrule
			 FP and FN &$\E \left[\var [\ell(h,z) \mid y]\right]$%\\$p(y=0) \var [\ell(h,z) \mid y=0] + p(y=1)\var [\ell(h,z) \mid y=1]$}
			 	\\
			\bottomrule
	\end{tabular}}
	\vspace{0.2cm}
	\caption{\label{tab:different_losses}Different objective variance to be used for different purposes. 
	If no outcome is favorable to another we use OM, if one outcome is favorable to another we use FP or FN (equal opportunity).
	We can also penalize both of these variances at the same time.}
\end{table}

==> different_regularizer.tex <==
\begin{table*}
	\centering
	\scalebox{0.8}{
	\begin{tabular}{llll}
		\toprule
		\bf Loss variance & \bf Formula & \bf Protected groups & \bf Examples on Income dataset\\ \midrule
			Group  & $\max_i \var [\ell \mid A_i]$ & $\sG^*_{A_i}$: Sensitive coarse groups (groups defined on $A_i$) & women\\
			Subgroup  & $\var [\E [\ell \mid A]]$& $\sG^*_A$: Sensitive fine groups (groups defined on $A$) & non white women\\
			Individual & $\var [\ell]$& 
			$\sG^*$: All groups (groups defined on $\sX$)& non white married women\\
			\bottomrule
	\end{tabular}}
	\caption{\label{tab:different_regularizers} Different loss variances and the groups that can be protected by bounding them.}
\end{table*}

==> framework.tex <==

%\paragraph{Evaluating fairness of a predictor.} Theorem \ar{fill number} of \cite{maurer2009empirical}
%shows that variance generalizes making the empirical variance of the loss on the training data
%an unbiased estimate of the fairness of a predictor.

\subsection{Loss variance and guarantees on the loss of any group}
Most current fairness notions are based on identifying \emph{groups} in the population
and (approximately) equalizing some property (like false positive rate) across these groups
and the overall population (e.g., \citep{calders2009building,zliobaite2015relation,hardt2016}). Our proposed loss variance on the other hand, approximately
equalizes the loss of an average \emph{individual} to the population loss. The individual based loss variance and group notions are indeed related, as we show next.

We denote a group by group indicator $g \in \sX \times \sY \mapsto \{0, 1\}$ such that $g(z) = 1$ if individual $z$ is in
the group and $0$ otherwise. We also denote $\ell(h, z)$ by $\ell$ for brevity in notation.
\begin{definition}[Group-unfairness]
For a set of groups $\sG$, we define the group-unfairness $U(\sG)$ as the worst-case difference in the loss of a group in $\sG$ and population loss. 
\begin{align*}
  \label{eqn:group-unfairness}
  U(\sG) &\eqdef \max \limits_{g \in \sG} \E[g(z)]  \Big( \E[ \ell \mid g(z)=1] -  \E[\ell] \Big)^2.
\end{align*}
\end{definition}
Let $\sG^\star$ be the set of all measurable binary functions on $\sX \times \sY$. $\sG^\star$ contains group indicators corresponding to \textit{all} groups in the population. 

Proposition~\ref{prop:varToGroup} and \ref{prop:groupToVar} together show that the loss variance is a close estimate of the group-unfairness for the set of all groups $U(\sG^\star)$.
\begin{restatable}{proposition}{propVarToGroup}
  \label{prop:varToGroup}
  Consider a predictor $h$ with some loss function $\ell$. Suppose the loss variance is less than $\gamma^2$.
  Then the group unfairness of the predictor for the set of all groups,
  \vspace{-10pt}
  \begin{align}
    U(\sG^\star) \leq \gamma^2. 
  \end{align}
\end{restatable}
%%%%%%%%%%%%%%%%%%%%%%% Move to appendix %%%%%%%%%%%%%%%%
\begin{comment}
\begin{sproof} From law of total variance we know:
	$\var[ \E[\ell(h, z) \mid g]] \leq \E[\var[\ell(h, z) \mid g]] + \var[ \E[\ell(h, z) \mid g]] = \var[\ell(h, z)] \leq \gamma^2$.
	We then by some simple algebra show $U(\sG^\star) \leq  \var[\E[ \ell(h, z) \mid g]]$.
\end{sproof}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-10pt}
In particular, the proposition says that for groups where $\E[g(z)] \geq \alpha$, 
the average loss within $g$ is bounded by a constant $\frac{\gamma}{\sqrt{\alpha}}$ from the population loss.
Therefore, bounding the loss variance protects all large groups. 
Next, we show the reverse implication that if the loss variance of the predictor is large,
then there exists a group with the loss far from the population loss (equivalently when $U(\sG^\star)$ is large).
This shows that
variance is a close estimate of $U(\sG^\star)$.
\begin{restatable}{proposition}{propGroupToVar}
	\label{prop:groupToVar}
	For any predictor $h$, with loss function $0 \le \ell \le L$, $\gamma \le L$ the following holds:
	\begin{align}
	\label{eqn:tight2} 
	\var[\ell] \le \gamma^2\left(2+4\ln\left(\frac{L}{\gamma}\right)\right) \implies U(\sG^\star) \le \gamma^2
	\end{align}
\end{restatable}

\begin{sproof}
  The loss variance provides an upper bound on the probability of a point having a loss $\geq u$ for any $u\ge0$. 
  We can use this upper bound to show that when there is a group with a large loss, the variance cannot be too small
  (See Appendix~\ref{sec:appendix} for details).
\end{sproof}
\input{variance_figure}
\subsection{Fairness in the presence of sensitive features}
\label{sec:sensitive }
In some cases, we are interested in only ensuring fairness with respect to
certain legally ``sensitive '' features like race, gender or citizenship status.
Formally, let $A$ denote the sensitive features of individuals. For example, $A = $ [race, gender $\hdots$]. Since we are only interested in groups
defined on $A$, we condition on $A$ and minimize the following \textit{subgroup loss variance}:
\begin{align}
\label{eqn:expLossVariance}
\var [ \E[\ell \mid A ] ] &= \E \large [  \big(\E[\ell \mid A] - \E[ \ell] \big)^2 \large ].
\end{align}
In other words, we pool in the losses of people who have the same sensitive features $A$
and then compute the variance across different values of the sensitive features. 
This notion is less restrictive than just loss variance because it ignores fluctuations in the losses of individuals who have identical sensitive features.
\reffig{withAndWithoutProtectedAttributes} shows the difference between simple loss variance and subgroup loss variance defined over sensitive features.
%%%%%%%%%%%%% It's already explained beneath caption %%%%%%%%%%%%%%
\begin{comment}
If we considered simple loss variance, the predictor would be unfair because it has a higher loss on the group of people with caps. However, if we were only interested in the sensitive features color and height, we would consider the predictor fair because the people with caps are evenly distributed across the groups defined on the sensitive features; the expected loss variance over these features is small.
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Since we are only interested in groups based on sensitive features, let's define $\sG^\star_A$ to be the set of all measurable binary functions on $A \mapsto \{0, 1\}$.
Proposition~\ref{prop:varToGroup} and~\ref{prop:groupToVar} hold with the set $\sG^\star$ replaced with $\sG_A^\star$.
In other words, subgroup loss variance is a close estimate of the group unfairness over the set of all groups defined on sensitive features. We provide the formal statements in \refcor{protected_group} in the Appendix.
%%%%%%%%%%%%%%%%%%% Move to appendix %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%xs
\begin{comment}
\begin{restatable}{corollary}{propProtected}
  \label{cor:sensitive_group}
  Consider a predictor $h$ with some loss function $\ell$. The following holds,
  \begin{align}
  \label{eqn:way1p}
   \nonumber \var[\E[\ell\mid A]] &\le \gamma^2 \implies\\ U(\sG^\star_A) &\leq \gamma^2, 
  \end{align}
 And conversely, if $0 \le \ell \le L$ then for any $\gamma \le L$ we have:
 	\begin{align}
 	\label{eqn:tightp}
 	\nonumber U(\sG^\star_A) &\leq \gamma^2 \\
 	\implies \var[\E[\ell\mid A]] &\le 2\gamma^2\left(1+2\ln\left(\frac{L}{\gamma}\right)\right)
 	\end{align}
\end{restatable}
The proof is essentially the same as that of Proposition~\ref{prop:varToGroup} and \ref{prop:groupToVar}, where we condition on sensitive features
at each step.
\end{comment} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Fairness in the presence of preferential outcomes}
%% \fk{can u change the text so it would be more consistent with the table? 
%% The table just says positive people should have similar loss in different groups.}
%% \fk{you can add a paragraph that we can define different losses as well}
\label{sec:conditional}
In some applications, there is a clear prefered outcome. In this case, different types of errors (false positive vs. false negatives) have different effect. For example, in the case of loan applications, fairness notions are concerned with eligible loan applications which were rejected. Here, we only penalize $\var[\ell \mid y = 1]$.
Similarly, for crime recidivism, we penalize $\var[\ell \mid y = 0]$. However, in applications like recommender systems where there is no prefered outcome, we penalize $\var[\ell]$.
%% The choice of the loss whose variance we minimize determines the type of fairness obtained.
%% Previous work has typically focused on a particular type of fairness, for example equalizing false positive/false negative rates.  In our work, we allow greater flexibility by allowing different losses to be incorporated. 
%% For example, consider the application of deciding whether to accept a loan application. There is a universally advantaged outcome of accepting the loan application. In this case, we penalize the variance of the false negative loss, as we want to ensure that eligible loan applications from all groups are equally considered. This is also referred to as equalized opportunity in \cite{hardt2016}.
%% Similarly, for the application of predicting crime recidivism, we choose the false positive loss.
%% For an application like recommender systems where there is no universally favored outcome, both types of errors (false positive and false negative) have to be controlled (equalized odds of \cite{hardt2016}). 
%% Additionally, we could also consider different losses that capture domain information appropriately. 
%% \input{different_loss}
%% \reftab{different_losses} contains the explicit regularization term imposed by considering the different losses. 




==> impossibility.tex <==
Unfortunately, it is impossible to provide equal protection for all groups with positive measure.
To see this, note that
group unfairness (\refdef{groupUnfairness}) implies lower and upper bounds on the expected loss of any group $g$ whose weight $w(g) > 0$:
\begin{align}
\E [\ell] - \frac{U(w)}{w(g)} \le \E [\ell \mid g] \le \E [\ell] + \frac{U(w)}{w(g)}
\end{align}

If all groups with positive measure are weighted equally ($w(g) = \1[\E[g] > 0]$), then $U(w)\le \epsilon$ implies the loss of any group $g$ with positive measure is bounded between $\E [\ell] - \epsilon$ and $\E [\ell] + \epsilon$.
For a bounded loss $0 \le \ell \le 1$, we call $\epsilon$ a non-trivial upper bound for $U(w)$ if $[0,1] \not\subseteq [\E [\ell] - \epsilon, \E{[\ell]+\epsilon}]$, i.e., the bound of $\epsilon$ on $U(w)$ provides
non-trivial information about the loss of groups.
In the following, we show that it is impossible to provide a non-trivial upper bound for $U(w)$ given finite training examples.

%some things to note
%1) \ell being trivial e.g. return 0 indipendent of X and h
%2) h being trivial e.g. return 0.5 for everyone.
%3) \ell should only be a function of z and h(x) otherwise it can look at the loss of all other point
%4) we don't care about support of X be small (e.g. only one point) since we assume |Y| >=2.



We call $(\ell, h)$ non-degenerate if there are some $z \in \sZ$ such that $\ell (h,z) = \epsilon$ and there are some $z'$ such that $\ell(h,z') = 1-\epsilon'$.
Intuitively if the classifier and loss function are not degenerate there should be some part of the input space that classifier can correctly classify and get low loss and we flip the label on those areas then the classifier should get high loss.
For some degenerate examples, assume loss function return $0$ independent of $h$ or $h$ return a constant and loss compute the $\ell(h,z)=|y-h(z)=0.5$ everywhere.
Intuitively, there are always some parts of input that a classifier have high loss there and if that group/part is really small it is possible that for any  given $n$ i.i.d. samples $\sP$, no samples is belong to that group.

We now show given \emph{any} $n$ i.i.d. examples from a distribution $\sP$ it is impossible to provide a non-trivial guarantee for $U(w)$
\begin{restatable}{proposition}{impossibility}
	\label{prop:impossibility} 
	For a predictor $h$ with loss function $0\le \ell\le 1$, if $w(g)=\1[\E [g] > 0]$, 
	given any $n$ i.i.d. samples from $\sP$, there is no non-trivial $\epsilon < \max (\E [\ell], 1-\E [\ell])$ and $\delta < 1$ such that $\pr [U(w) \le \epsilon] > 1-\delta$.
	\pl{are these quantifiers right?}
\end{restatable}

\begin{proof}
	If $U(w) \ge \max (\E [\ell], 1-\E[\ell])$ then obviously there is no $\epsilon$ such that $U(w) \le \epsilon$.
	%
	Now let assume actually $U(w) \le \max (\E [\ell], 1-\E[\ell])$, without loss of generality assume $1 \notin (\E [\ell], 1-\E[\ell])$. 
	Since we assume $(\ell, \sH)$ is not obvious then there exists some $z^\star$ such that $\ell (h,z) =1$.
	We now define a new distribution $\sP_2$ and show 
	
	\begin{align}
	\sP_2 = 
	\begin{cases}
	\sqrt[n]{\delta} \sP(z) & z\neq z^\star\\
	1-\sqrt[n]{\delta} & z\neq z^\star
	\end{cases}
	\end{align}
	Therefore with probability of $\delta$ the $n$ samples might come from  
\end{proof}

Similarly, 





\refprop{impossibility} shows that we cannot protect all groups equally
since statistically, we cannot control the combinatorial number of tiny groups using finite samples.
It seems therefore natural to consider a weighting function $w$ that assigns smaller weight to smaller groups.
But what is an appropriate weighting function?
%intuition behind \sqrt{E[g]}
%Every group $g$ will have a confidence bound as follows:
%\begin{align}
%\label{eqn:conf_intervals}
%\E [\ell] - \frac{U(w)}{w(g)} \le \E [\ell \mid g] \le \E [\ell] + \frac{U(w)}{w(g)}
%\end{align}
%Having $w(g) = \sqrt{\E [g]}$ will make the confidence bound in line with Hoeffding or Bennet confidence interval.
%section 3
%section 4
%% In Section~\ref{sec:fairness_CLV}, we show that controlling different variations of loss variance cause protection for groups according to different weighting functions.
%% In particular, in \refsec{fairness_CLV} we show controlling ``coarse loss variance'' causes protection only on groups defined on sensitive attributes.

==> impossibility_proof_sketch.tex <==
\begin{sproof}
	Consider distribution $p_1$ such that $\mwld (w^0, \ell, h)$ (\refdef{mwld}) is less than $\half$ regarding to $p_1$.
	Let $z_0$ and $z_1$ be data points with loss $0$ and $1$ respectively.
	We construct a new distribution $p_2$ as follows: for $\eta = 1-\sqrt[n]{\frac{\delta}{1-\delta}}$ 
	with probability $(1 - \eta)$, $z \sim p_1$ and $z = z_0$ and $z = z_1$ with probability $\frac{\eta}{2}$ each.
	$\mwld(w^0, \ell, h)$ of $p_2$ is greater than $\half$.
	We then prove it is impossible to accurately estimate both distributions (see \ref{sec:appendix} for details).
\end{sproof}
%\begin{sproof}
%Assume for $w_0$ auditor $\sA$ exists.
%Consider distribution $p_1$ such that its weighted group unfairness is less than $\half$.
%\begin{align*}
%U_1 &\eqdef \max \limits_{g \in \sG, \E[g] > 0} \Big | \E_{p_1}[\ell(h, z) \mid g(z) = 1] -  \E_{p_1}[\ell(h, z)] \Big| 
% < \half ~~ \text{(By assumption)}.
%\end{align*}          
%We can construct a new distribution $p_2$ as follows: for $\eta = 1-\sqrt[n]{\frac{\delta}{1-\delta}}$ 
%with probability $(1 - \eta)$, $z \sim p_1$ and $z = z_\text{high}$ and $z = z_\text{high}$ with probability $\frac{\eta}{2}$ each.
%The group unfairness for this distribution $U_2$ is defined analogous to $U_1$ above.
%By the existence of groups $g_\text{high}, g_\text{low}$ corresponding to the singletons $z_\text{high}$ and $z_\text{low}$ with $\E[g_\text{high}] = \E[g_\text{low}] = \frac{\eta}{2} > 0$,
%we have $U_2 \ge \frac{1}{2}$. 
%
%
%Let $\gamma_1$ and $\gamma_2$ denote two random variables corresponding to the estimates of auditor for $U_1$ and $U_2$ respectively; 
%set $\epsilon = \frac{\half - U_1}{2}$, with some substitutions (see Appendix~\ref{sec:appendix}) we have:
%
%\begin{align}
%\pr (|\gamma_2 - U_2 | > \epsilon) 
%%&\ge \pr (\gamma_2 - U_2 < -\epsilon)\\
%%&= \pr (\gamma_2 < U_2 - \epsilon)\\
%%&\ge \pr (\gamma_2 < \half - \epsilon )\\
%%&\ge \pr (\gamma_2 < \half - (\frac{\half - U_1}{2}))\\
%%&= \pr (\gamma_2 \le U_1+ \epsilon)\\
%%&\ge \pr (|\gamma_2 - U_1| \le \epsilon)\\
%&\ge (1-\eta)^n\pr (|\gamma_1 - U_1| \le \epsilon)
%%&> (1-\eta)^n(1-\delta) \\
%%&=\p {1-\p {1-\sqrt[n]{\frac{\delta}{1-\delta}}}}^n (1-\delta) \\
%> \delta
%\end{align}
%Which contradicts the assumption that $\sA$ is an auditor and should guarantee $\pr \left[ |\gamma_2 - U_2| > \epsilon \right] \le \delta$.
%\end{sproof}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> mwld_different_k_all.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.3\textwidth]{images/new/mwld_different_k_all.pdf}
	\caption{$\mwld(\wk)$ for different values of $k$ in different datasets.
	Dashed lines are corresponding to the train set and solid lines are corresponding to the test set.}
\end{figure}

%\begin{figure}
%	\centering
%	\includegraphics[width=\textwidth]{images/new/group_fairness_interpretation_compass5.pdf}
%	(a)\hspace{0.3\textwidth}(b)\hspace{0.3\textwidth}(c)
%	\caption{
%	For each predictor we can compute the worst loss discrepancy for any group size (a) shows the worst loss discrepancy for different group sizes in COMPAS\_5 dataset.
%	As shown in \reffig{different_k_guarantees} $\mwld(\wk)$ provides an upper bound guarantee for all groups; for smaller $k$ this upper bound is more restrictive and needs all the loss discrepancy (independent of their size) be under this graph.
%	Each $k$ has different curvature in (b) we show how did we find curvature that are upper bounded for the black curve. As $k$ decreases means it need similar guarantees for all group therefore $\mwld(\wk)$ has larger values. 
%	Another way to look at this is shown in (c) where instead of looking the whole curve we multiply each point by $\E [g]^k$ and compute the maximum. }
%\end{figure}
